Slim DensePose: Thrifty Learning from Sparse Annotations and Motion Cues

DensePose supersedes traditional landmark detectors by densely mapping image pixels to body surface coordinates. This power, however, comes at a greatly increased annotation time, as supervising the model requires to manually label hundreds of points per pose instance. In this work, we thus seek methods to significantly slim down the DensePose annotations, proposing more efficient data collection strategies. In particular, we demonstrate that if annotations are collected in video frames, their efficacy can be multiplied for free by using motion cues. To explore this idea, we introduce DensePose-Track, a dataset of videos where selected frames are annotated in the traditional DensePose manner. Then, building on geometric properties of the DensePose mapping, we use the video dynamic to propagate ground-truth annotations in time as well as to learn from Siamese equivariance constraints. Having performed exhaustive empirical evaluation of various data annotation and learning strategies, we demonstrate that doing so can deliver significantly improved pose estimation results over strong baselines. However, despite what is suggested by some recent works, we show that merely synthesizing motion patterns by applying geometric transformations to isolated frames is significantly less effective, and that motion cues help much more when they are extracted from videos.

==> fig-blur.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/blur_.pdf}
\caption{Examples from DP-Track with extreme motion blur. First row: DP-COCO, second row: DP-(COCO+Track), third row: DP-(COCO+Track)}\label{fig:blur}
\end{figure}

==> fig-reduced.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=.88\linewidth]{figures/reduced.pdf}\vspace*{-1mm}
%\caption{\textbf{Reduced supervision} for DensePose.}\label{fig:reduced}
\end{figure}

==> fig-splash.tex <==
\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/teaser_v2.pdf}\\
%{\scriptsize \hspace*{6mm} input \hspace*{9mm} DensePose-COCO \hspace*{1mm} \textbf{DensePose-Track} \hspace*{3mm} \textbf{DensePose-Slim}}\vspace*{1mm}
\caption{DensePose trained on COCO (second column) tends to fail on particularly challenging poses affected by significant blur, low resolution, and unusual geometry. We introduce a more challenging DensePose-Track dataset (third column) collected from videos and show how motion cues can be used to amplify the efficacy of its annotations, obtaining improved results (last column) in these challenging scenarios.}\label{f:splash}
% \caption{Compared to training on COCO (column 2), the introduced DensePose-Track gives better results with motion (column 3) which are improved by further leveraging motion cues in DensePose-Slim (column 4)}\label{f:splash}
\end{figure}

==> tab-unknown.tex <==
\begin{table}[!htb]
\centering
\begin{tabular}{|l|c|c|c|c|}%c|c|}
\hline
$\vphantom{\rule{0mm}{3.5mm}}$
\hspace*{8.8mm}\emph{Data} & \hspace*{0.1mm}5 cm\hspace*{0.1mm}&  \hspace*{0.1mm}10 cm\hspace*{0.1mm}&  \hspace*{0.1mm}20 cm\hspace*{0.1mm} \\%& \emph{$\mathbf{FR}_{10}$} & \emph{$\mathbf{FR}_{30}$} \\
\hline\hline
\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Test-COCO}}\\ \hline
  train-COCO & 55.78 & 82.34 & 92.55\\
train-(COCO+PoseTrack) &  55.27 & 82.05 & 92.37\\%& 0.57& 0.42 \\
train-PoseTrack &  20.34 & 41.24 & 57.29 \\%& 0.57& 0.42 \\
train-COCO[size:Posetrack] &  46.36 & 73.26 & 85.72 \\%& 0.57& 0.42 \\
\hline\hline
8stack-train-COCO & 58.23 & 84.07 & 93.58  \\
\hline
\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Test-PoseTrack}}\\ \hline
train-COCO & 42.55 & 69.50 & 82.74 \\
  train-(COCO+PoseTrack) &  41.76 & 69.94 & 83.60 \\%& 0.57& 0.42 \\
  train-PoseTrack &  21.06 & 42.94 & 59.54  \\
train-COCO[size:Posetrack] &  33.67 & 58.79 & 73.45\\ %& 0.57& 0.42 \\
\hline\hline
1stack-train-COCO & 34.47 & 61.93 & 76.88  \\
2stack-train-COCO & 42.55 & 69.50 & 82.74  \\
3stack-train-COCO & 43.84 & 70.82 & 83.64  \\
4stack-train-COCO & 44.12 & 71.19 & 83.91  \\
  5stack-train-COCO & 44.87 & 71.52 & 83.84  \\
6stack-train-COCO & 44.89 & 71.52 & 83.71  \\
%(E06) 7stack-train-COCO & - & - & - & \\
  8stack-train-COCO & 44.28 & 70.75 & 83.08  \\
\hline
\end{tabular}
\vspace*{2mm}
\caption{R.}
\end{table}

==> tab-weakify-2.tex <==
\begin{table}[!htb]
\centering
\begin{tabular}{|l|c|c|c|}%c|c|}
\hline
$\vphantom{\rule{0mm}{3.5mm}}$
\hspace*{8.8mm}\emph{Data} & \hspace*{0.1mm}5 cm\hspace*{0.1mm}&  \hspace*{0.1mm}10 cm\hspace*{0.1mm}&  \hspace*{0.1mm}20 cm\hspace*{0.1mm} \\%& \emph{$\mathbf{FR}_{10}$} & \emph{$\mathbf{FR}_{30}$} \\
\hline\hline
%\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
%\textit{TPS-COCO}}\\ \hline
%Baseline & 55.78 & 82.34 & 92.55 \\
%GP propagation & --55.43 & 82.44 & 92.80 \\
%Equivariance-warpfeat & --44.00 &  74.10 & 88.35 \\
%Equivariance-dowarp & --XX &  XX & XX \\
%GT propagation + equiv &  52.47 & 80.84 & 92.09 \\%& 0.57& 0.42 \\
%\hline\hline
%\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
%\textit{TPS-COCO (test posetrack)}}\\ \hline
%Baseline & 42.55 & 69.50 & 82.74 \\
%(A00) Baseline & 43.36 & 70.33 & 83.34 & 3907084, 3909184, wrong baseline\\
%GP propagation & XX &  XX & XX \\
%Equivariance & XX &  XX & XX \\
%GT propagation + equiv &  XX & XX & XX \\%& 0.57& 0.42 \\
%\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
%\textit{Warpfeat-COCO[size:Posetrack]}}\\ \hline
%Baseline & XX &  XX & XX \\
%GP propagation & XX & XX & XX \\
%Equivariance & XX &  XX & XX \\
%GT propagation + equiv &  XX & XX & XX \\%& 0.57& 0.42 \\
%\hline\hline
\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{TPS}}\\ \hline
Baseline & 21.06 & 42.94 & 59.54\\
GT propagation & 22.33 &  45.30 & 62.08\\
Equivariance & 21.57 & 44.17 & 61.27 \\
GT propagation + equiv &  22.41 & 45.53 & 62.71 \\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Flow}}\\ \hline
Baseline & 21.06 & 42.94 & 59.54\\
%Only propagated & 30.80 &  55.44 & 70.66\\
GT propagation & 32.85 & 60.07 & 75.95\\
Equivariance & 23.12 &  45.85 & 62.22\\
GT propagation + equiv &  XX & XX & XX \\%& 0.57& 0.42 \\
\hline\hline
%\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
%\textit{Warpfeat/warpflow-PoseTrack}}\\ \hline
% Baseline & 21.06 & 42.94 & 59.54 \\
%GP propagation & XX &  XX & XX \\
%Equivariance & XX & XX & XX \\
%GT propagation + equiv &  XX & XX & XX \\%& 0.57& 0.42 \\
%\hline\hline
\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{TPS-Posetrack-init COCO}}\\ \hline
Baseline & 44.22  & 71.78 & 84.54  \\
GT propagation & 44.57 & 72.06 & 84.70  \\
  Equivariance & 44.70 & 72.13 & 84.75\\
GT propagation + equiv & 44.78 & 72.26 & 84.82 \\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Flow-PoseTrack-init COCO}}\\ \hline
Baseline & 44.22  & 71.78 & 84.54\\
GT propagation & 45.98 & 73.57 & 86.11 \\
Equivariance & - &  - & - \\
GT propagation + equiv &  XX & XX & XX \\%& 0.57& 0.42 \\
\hline\hline
%\multicolumn{4}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
%\textit{Warpfeat/warpflow-PoseTrack-init COCO}}\\ \hline
%Baseline & 44.22  & 71.78 & 84.54   \\
%GP propagation & - & - & - \\
%Equivariance & - & -  & - \\
%GT propagation + equiv & - & - & - \\%& 0.57& 0.42 \\
\end{tabular}
\vspace*{2mm}
\caption{Tested on Posetrack (?).} 
\label{fig:weakify}
\end{table}


==> tab-weakify-3.tex <==
\begin{figure}[!htb]
\centering
\begin{tabular}{|l|c|c|c|c|}%c|c|}
\hline
$\vphantom{\rule{0mm}{3.5mm}}$
\hspace*{8.8mm}\emph{Data} & \hspace*{0.1mm}5 cm\hspace*{0.1mm}&  \hspace*{0.1mm}10 cm\hspace*{0.1mm}&  \hspace*{0.1mm}20 cm\hspace*{0.1mm} & job id \\%& \emph{$\mathbf{FR}_{10}$} & \emph{$\mathbf{FR}_{30}$} \\
\hline\hline
(A00) Full dataset & 55.78 & 82.34 & 92.55 & 3907084\\ 
%(A01) Only masks & XX &  XX & XX & 3909078 \\ 
(A02) Only segmentation (+I) & 3.53 & 13.25 & 48.21 & \st{3909079}\\ \hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Subset of images}}\\ \hline
(A03) 50\% &  52.49 & 79.45 & 90.40 & \st{3908864}\\%& 0.57& 0.42 \\
(A04) 20\% &  47.10 & 74.06 & 86.27 & \st{3909046}\\%& 0.57& 0.42 \\
(A05) 10\% &  41.51 & 68.04 & 81.70 & \st{3909047}\\%& 0.57& 0.42 \\
(A06) 5\% &  36.27 & 64.58 & 79.93 & \st{3909047}\\%& 0.57& 0.42 \\
(A07) 1\% &  14.11 & 32.06 & 50.21 & \st{3909049}\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Subset of images}}\\ \hline
(A18) all masks + 50\% &  53.50 & 80.29 & 90.86 & 3923705\\%& 0.57& 0.42 \\
(A19) all masks + 20\% &  49.26 & 76.47 & 88.21 & 3923704 \\%& 0.57& 0.42 \\
(A20) all masks + 10\% &  44.71 & 72.38 & 85.22 & 3923703\\%& 0.57& 0.42 \\
(A21) all masks + 5\% &  40.80 & 69.04 & 83.15 & 3923702 \\%& 0.57& 0.42 \\
(A22) all masks + 1\% &  36.16 & 66.59 & 83.14 & 3923701\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Subset of images - warpfeat}}\\ \hline
(A18) 50\% &  - & - & - & 3923705\\%& 0.57& 0.42 \\
(A19) 20\% &  - & - & - & 3923704 \\%& 0.57& 0.42 \\
(A20) 10\% &  - & - & - & 3923703\\%& 0.57& 0.42 \\
(A21) 5\% &  - & - & - & 3923702 \\%& 0.57& 0.42 \\
(A22) 1\% &  - & - & - & 3923701\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Subset of images - warpfeat + GT-prop}}\\ \hline
(A23) 50\% & - & - & - & 3923710\\%& 0.57& 0.42 \\
(A24) 20\% & -  & - & - & 3923709\\%& 0.57& 0.42 \\
(A25) 10\% & - & - & - & 3923708\\%& 0.57& 0.42 \\
(A26) 5\% & - & - & - & 3923707\\%& 0.57& 0.42 \\
(A27) 1\% & - & - & - & 3923706\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Subset of points}}\\ \hline
(A13) all masks + 50\% &  54.06 & 81.24 & 91.92 & 3907859\\%& 0.57& 0.42 \\
(A14) all masks + 20\% &  52.79 & 80.39 & 91.42 & 3909077\\%& 0.57& 0.42 \\
(A15) all masks + 10\% &  50.58 & 78.65 & 90.23 & 3907800\\%& 0.57& 0.42 \\
(A16) all masks + 5\% &  47.68 & 76.34 & 88.86 & 3907658\\%& 0.57& 0.42 \\
(A17) all masks + 1\% &  37.65 & 68.25 & 84.37 & 3908953\\%& 0.57& 0.42 \\
\hline
\end{tabular}
\vspace*{2mm}
\caption{Reducing amount of direct supervision.} 
\label{fig:weakify}
\end{figure}

\begin{figure*}[!htb]
\centering
\begin{tabular}{|l|c|c|c|c|}%c|c|}
\hline
$\vphantom{\rule{0mm}{3.5mm}}$
\hspace*{8.8mm}\emph{Data} & \hspace*{0.1mm}5 cm\hspace*{0.1mm}&  \hspace*{0.1mm}10 cm\hspace*{0.1mm}&  \hspace*{0.1mm}20 cm\hspace*{0.1mm} & job id\\%& \emph{$\mathbf{FR}_{10}$} & \emph{$\mathbf{FR}_{30}$} \\
\hline\hline
(A00) baseline & 55.78 & 82.34 & 92.55 & 3907084, 3916430\\
(B00) all masks + 100\% + kp & 44.79 &  XX & XX & 3916049\\
(B01) all masks + 1\% + kp &  XX & XX & XX & 3916048, 3918126 \\%& 0.57& 0.42 \\
(B02) all masks + kp &  36.60 & 63.03 & 76.81 & \st{3908948}, \st{3909188}, 3918123  \\%& 0.57& 0.42 \\
(B03) all masks + kp + warpfeat &  XX & XX & XX & 3908949, 3909187, 3918125\\%& 0.57& 0.42 \\
\hline \hline
(B04) all masks + kp + VAR &  XX & XX & XX &\\%& 0.57& 0.42 \\
(B05) all masks + kp + EIGEN &  XX & XX & XX &\\%& 0.57& 0.42 \\
(B06) all masks + kp + NEG &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline
\end{tabular}
\vspace*{2mm}
\caption{Reducing amount of direct supervision + keypoints.} 
\label{fig:weakify}
\end{figure*}


==> tab-weakify-4.tex <==
\begin{figure*}[!htb]
\centering
\begin{tabular}{|l|c|c|c|c|}%c|c|}
\hline
$\vphantom{\rule{0mm}{3.5mm}}$
\hspace*{8.8mm}\emph{Data} & \hspace*{0.1mm}5 cm\hspace*{0.1mm}&  \hspace*{0.1mm}10 cm\hspace*{0.1mm}&  \hspace*{0.1mm}20 cm\hspace*{0.1mm} & job id\\%& \emph{$\mathbf{FR}_{10}$} & \emph{$\mathbf{FR}_{30}$} \\
\hline\hline
(A00) baseline & 55.78 & 82.34 & 92.55 & 3907084, 3916430\\
(B00) all masks + 100\% + kp & 44.79 &  XX & XX & 3916049\\
(B01) all masks + 1\% + kp &  XX & XX & XX & 3916048, 3918126 \\%& 0.57& 0.42 \\
(B02) all masks + kp &  36.60 & 63.03 & 76.81 & \st{3908948}, \st{3909188}, 3918123  \\%& 0.57& 0.42 \\
(B03) all masks + kp + warpfeat &  XX & XX & XX & 3908949, 3909187, 3918125\\%& 0.57& 0.42 \\
\hline \hline
(B04) all masks + kp + VAR &  XX & XX & XX &\\%& 0.57& 0.42 \\
(B05) all masks + kp + EIGEN &  XX & XX & XX &\\%& 0.57& 0.42 \\
(B06) all masks + kp + NEG &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline
\end{tabular}
\vspace*{2mm}
\caption{Reducing amount of direct supervision + keypoints.} \label{fig:weakify}
\end{figure*}


==> tab-weakify-5.tex <==
\begin{figure*}[!htb]
\centering
\begin{tabular}{|l|c|c|c|c|}%c|c|}
\hline
$\vphantom{\rule{0mm}{3.5mm}}$
\hspace*{8.8mm}\emph{Data} & \hspace*{0.1mm}5 cm\hspace*{0.1mm}&  \hspace*{0.1mm}10 cm\hspace*{0.1mm}&  \hspace*{0.1mm}20 cm\hspace*{0.1mm} & job id\\%& \emph{$\mathbf{FR}_{10}$} & \emph{$\mathbf{FR}_{30}$} \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-COCO}}\\ \hline
(A00) Baseline & 55.78 & 82.34 & 92.55 & 3907084, 3909163\\
(D01) GP propagation & --55.43 & 82.44 & 92.80 & 3909164, 3916439, 3916439, 3917855\\
(D02) Equivariance-warpfeat & --44.00 &  74.10 & 88.35 & 3909165 (early), 3917145, 3917678, 3917786\\
(D02) Equivariance-dowarp & --XX &  XX & XX & 3917842\\
(D03) GT propagation + equiv &  52.47 & 80.84 & 92.09 & 3909166 (early)\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-COCO (test posetrack)}}\\ \hline
(A00) Baseline & 42.55 & 69.50 & 82.74 & 3907084, 3909184\\
%(A00) Baseline & 43.36 & 70.33 & 83.34 & 3907084, 3909184, wrong baseline\\
(D16) GP propagation & XX &  XX & XX & 3909179\\
(D17) Equivariance & XX &  XX & XX & 3909177\\
(D18) GT propagation + equiv &  XX & XX & XX & 3909176\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-COCO[size:Posetrack]}}\\ \hline
(C02) Baseline & XX &  XX & XX & 3909046\\
(D04) GP propagation & XX & XX & XX & 3909181 (early)\\
(D05) Equivariance & XX &  XX & XX & 3909182\\
(D06) GT propagation + equiv &  XX & XX & XX & 3909183\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-Posetrack}}\\ \hline
(C01) Baseline & 21.06 & 42.94 & 59.54 & 3909131, 3909168\\
(D07) GP propagation & 22.33 &  45.30 & 62.08 & 3909174\\
(D08) Equivariance & 21.57 & 44.17 & 61.27 & 3909173, 3917677\\
(D09) GT propagation + equiv &  22.41 & 45.53 & 62.71 & 3909172\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpflow-PoseTrack}}\\ \hline
(C01) Baseline & 21.06 & 42.94 & 59.54 & 3909131, 3909168\\
(D19) Only propagated & 30.80 &  55.44 & 70.66 & 3915997, 3915998\\
(D10) GP propagation & 32.85 & 60.07 & 75.95 & 3915999, devfair-ik\\
(D11) Equivariance & 23.12 &  45.85 & 62.22 & 3915992, fn 3916443, 3917217\\
(D12) GT propagation + equiv &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat/warpflow-PoseTrack}}\\ \hline
(C01) Baseline & 21.06 & 42.94 & 59.54 & 3909131, 3909168, \st{devfair-nn}\\
(D13) GP propagation & XX &  XX & XX &\\
(D14) Equivariance & XX & XX & XX &\\
(D15) GT propagation + equiv &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-Posetrack-init COCO}}\\ \hline
(F00) Baseline & 44.22  & 71.78 & 84.54 & \\
(G00) GP propagation & 44.57 & 72.06 & 84.70 & \\
(G01) Equivariance & 44.70 & 72.13 & 84.75 & -\\
(G02) GT propagation + equiv & 44.78 & 72.26 & 84.82 & \\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpflow-PoseTrack-init COCO}}\\ \hline
(F00) Baseline & 44.22  & 71.78 & 84.54 &\\
(F01) GP propagation & 45.98 & 73.57 & 86.11 & \\
(G04) Equivariance & - &  - & - & 3\\
(G05) GT propagation + equiv &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat/warpflow-PoseTrack-init COCO}}\\ \hline
(F00) Baseline & 44.22  & 71.78 & 84.54 &  \\
(G06) GP propagation & - & - & - &\\
(G07) Equivariance & - & -  & - &\\
(G08) GT propagation + equiv & - & - & - &\\%& 0.57& 0.42 \\
\end{tabular}
\vspace*{2mm}
\caption{Tested on Posetrack (?).} 
\label{fig:weakify}
\end{figure*}

==> tab-weakify-rebuttal.tex <==
\begin{figure*}[!htb]
\centering
\begin{tabular}{|l|c|c|c|c|}%c|c|}
\hline
$\vphantom{\rule{0mm}{3.5mm}}$
\hspace*{8.8mm}\emph{Data} & \hspace*{0.1mm}5 cm\hspace*{0.1mm}&  \hspace*{0.1mm}10 cm\hspace*{0.1mm}&  \hspace*{0.1mm}20 cm\hspace*{0.1mm} & job id\\%& \emph{$\mathbf{FR}_{10}$} & \emph{$\mathbf{FR}_{30}$} \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-COCO}}\\ \hline
(A00) Baseline & 55.78 & 82.34 & 92.55 & 3907084, 3909163\\
(D01) GP propagation & --55.43 & 82.44 & 92.80 & 3909164, 3916439, 3916439, 3917855\\
(D02) Equivariance-warpfeat & --44.00 &  74.10 & 88.35 & 3909165 (early), 3917145, 3917678, 3917786\\
(D02) Equivariance-dowarp & --XX &  XX & XX & 3917842\\
(D03) GT propagation + equiv &  52.47 & 80.84 & 92.09 & 3909166 (early)\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-COCO (test posetrack)}}\\ \hline
(A00) Baseline & 42.55 & 69.50 & 82.74 & 3907084, 3909184\\
%(A00) Baseline & 43.36 & 70.33 & 83.34 & 3907084, 3909184, wrong baseline\\
(D16) GP propagation & XX &  XX & XX & 3909179\\
(D17) Equivariance & XX &  XX & XX & 3909177\\
(D18) GT propagation + equiv &  XX & XX & XX & 3909176\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-COCO[size:Posetrack]}}\\ \hline
(C02) Baseline & XX &  XX & XX & 3909046\\
(D04) GP propagation & XX & XX & XX & 3909181 (early)\\
(D05) Equivariance & XX &  XX & XX & 3909182\\
(D06) GT propagation + equiv &  XX & XX & XX & 3909183\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-Posetrack}}\\ \hline
(C01) Baseline & 21.06 & 42.94 & 59.54 & 3909131, 3909168\\
(D07) GP propagation & 22.33 &  45.30 & 62.08 & 3909174\\
(D08) Equivariance & 21.57 & 44.17 & 61.27 & 3909173, 3917677\\
(D09) GT propagation + equiv &  22.41 & 45.53 & 62.71 & 3909172\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpflow-PoseTrack}}\\ \hline
(C01) Baseline & 21.06 & 42.94 & 59.54 & 3909131, 3909168\\
(D19) Only propagated & 30.80 &  55.44 & 70.66 & 3915997, 3915998\\
(D10) GP propagation & 32.85 & 60.07 & 75.95 & 3915999, devfair-ik\\
(D11) Equivariance & 23.12 &  45.85 & 62.22 & 3915992, fn 3916443, 3917217\\
(D12) GT propagation + equiv &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat/warpflow-PoseTrack}}\\ \hline
(C01) Baseline & 21.06 & 42.94 & 59.54 & 3909131, 3909168, \st{devfair-nn}\\
(D13) GP propagation & XX &  XX & XX &\\
(D14) Equivariance & XX & XX & XX &\\
(D15) GT propagation + equiv &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat-Posetrack-init COCO}}\\ \hline
(F00) Baseline & 44.22  & 71.78 & 84.54 & \\
(G00) GP propagation & 44.57 & 72.06 & 84.70 & \\
(G01) Equivariance & 44.70 & 72.13 & 84.75 & -\\
(G02) GT propagation + equiv & 44.78 & 72.26 & 84.82 & \\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpflow-PoseTrack-init COCO}}\\ \hline
(F00) Baseline & 44.22  & 71.78 & 84.54 &\\
(F01) GP propagation & 45.98 & 73.57 & 86.11 & \\
(G04) Equivariance & - &  - & - & 3\\
(G05) GT propagation + equiv &  XX & XX & XX &\\%& 0.57& 0.42 \\
\hline\hline
\multicolumn{5}{|c|}{$\vphantom{\rule{0mm}{3.5mm}}$ 
\textit{Warpfeat/warpflow-PoseTrack-init COCO}}\\ \hline
(F00) Baseline & 44.22  & 71.78 & 84.54 &  \\
(G06) GP propagation & - & - & - &\\
(G07) Equivariance & - & -  & - &\\
(G08) GT propagation + equiv & - & - & - &\\%& 0.57& 0.42 \\
\end{tabular}
\vspace*{2mm}
\caption{Tested on Posetrack (?).} 
\label{fig:weakify_rebuttal}
\end{figure*}
